PRIPEL: Privacy-Preserving Event Log Publishing Including Contextual Information

Event logs capture the execution of business processes in terms of executed activities and their execution context. Since logs contain potentially sensitive information about the individuals involved in the process, they should be pre-processed before being published to preserve the individuals' privacy. However, existing techniques for such pre-processing are limited to a process' control-flow and neglect contextual information, such as attribute values and durations. This thus precludes any form of process analysis that involves contextual factors. To bridge this gap, we introduce PRIPEL, a framework for privacy-aware event log publishing. Compared to existing work, PRIPEL takes a fundamentally different angle and ensures privacy on the level of individual cases instead of the complete log. This way, contextual information as well as the long tail process behaviour are preserved, which enables the application of a rich set of process analysis techniques. We demonstrate the feasibility of our framework in a case study with a real-world event log.

==> validation.tex <==

\section{Validation}
\label{sec:validation}
In this section, we first demonstrate the feasibility of the PRIPEL framework by introducing a proof-of-concept implementation and applying it in a case study to a real-world event log (\autoref{sec:feasibility}). Afterwards, we discuss the framework's generalisability and limitations in \autoref{sec:discussion}.
\todo{Han: not sure if generalisability is the right word}



\subsection{Feasibility}
\label{sec:feasibility}


\subsubsection{Proof-of-Concept Implementation}
We implemented PRIPEL in Python and published our implementation under the MIT licence on Github\footnote{\url{https://github.com/samadeusfp/PRIPEL}}. Our implementation for differential privacy is based on the IBM library diffprivlib~\cite{holohan2019diffprivlib}.
 Additionally, we used PM4Py~\cite{berti2019process}
 and used its data structures for our implementation, to ensure compatibility with other approaches. Our implementation includes the PRIPEL specific parts such as the sequence enrichment component or a component that applies local differential privacy, but also a Python implementation of the differential private trace-variant query~\cite{mannhardt2019privacy}. 

\begin{table}
	\begin{tabularx}{\linewidth}{X X X X X X}
		\toprule
		Event Log &\# of Events & \# of Variants & \# of Case \\
		\midrule
		Sepsis  & 15,214 & 846 & 1,050  \\
		%
		%
		\bottomrule
	\end{tabularx}
	\caption{Event Logs Characteristics}
	\label{tab:datasets}
\end{table}

\todo{lift to additional subsections?}

\subsubsection{Case Study} We show the feasibility of our approach by applying \emph{PRIPEL} to a public real-world event log, the Sepsis event log~\cite{mannhardt2016sepsis}. \todo{Han: why did we choose this one?}
We show the event log characteristic in \autoref{tab:datasets}. In the case study we analyse if \emph{PRIPEL} is able to be performed in a reasonable time and if the framework is able to maintain utility in the event log.

For our case study we set the differential privacy guarantee parameter to $\epsilon=1.0$. We decided to opt for a the setting, where \emph{PRIPEL} throws away the unmatched, to ensure a better compatibility of our approach with the original log. Besides selecting the privacy guarantee $\epsilon$ our used trace-variant query~\cite{mannhardt2019privacy} can be tuned with two  parameters, $n$ and $k$, which influence the prefix-tree that the mechanism uses to generate a query result. 
With $n$ the maximum prefix-tree can be set.  While $k$ is used to prevent combinatorial explosion of potential prefixes, by limiting the expansion of the prefix-tree to prefixes with at least $k$ traces in their noisy count. We set $k=2$ and $N=30$ for our case study.

The runtime of \emph{PRIPEL} for the case study is shown in \autoref{tab:runtime}. The data clearly shows that most of the runtime comes from the sequence enrichment. However, the reason is the application of algorithm to find the the optimal assignment. Alternatively, a greedy strategy could be applied to reduce the runtime.




\begin{table}
	\begin{tabularx}{\linewidth}{X X X |X}
		\toprule
		TV-Query & Sequence Enrichment Matching & LDP & Total \\
		\midrule
		2s & 8m31s  & 38s & 9m14s  \\
		%
		%
		\bottomrule
	\end{tabularx}
	\caption{Runtime of \emph{PRIPEL} for the Sepsis log}
	\label{tab:runtime}
\end{table}


We used Apromore~\cite{la2011apromore} to analyse the anonymized event log and compare it with the original log. We retrieved several statistical measurements from both logs and compare them in table~\ref{tab:case_duration}. Based on the data it is obvious that the anonymized log consists of shorter traces, than the original log. The longest trace in the anonymized log consists of 30 events, while the longest trace in the original log consists of 370 events. However, we tried higher values for $N$ for the anonymized log, to enable longer trace, but noticed that this can lead to higher level of noise added. Since the prefixes of the original log get sparser the longer they get. Therefore, we decided against a higher value for $N$. However, we have still been able to obtain results close to the original value for 2 out of 4 metrics. Additionally, we would have been able to conclude that the average is far below the median. Therefore, we could conclude on the distribution of trace durations. Conclusively,  we can reason that an anonymized event logs allows us to gain useful insights about a business process.

\begin{table}
	\begin{tabularx}{\linewidth}{X X X X X}
		\toprule
		Log & Min & Max & Avg. & Median \\
		\midrule
		Original & 2min  & 1.2 years & 4.1 weeks & 5.4 days  \\
		Anonymized &  2min & 1.1 years & 2 weeks & 2 days \\
		%
		%
		\bottomrule
	\end{tabularx}
	\caption{Case Duration Measurements}
	\label{tab:case_duration}
\end{table}

In figure~\ref{fig:active_cases} we visualize the active cases over time for the Sepsis dataset, red denote the original event log, while blue represents the anonymized event log. We can see that the general trends of the log can be sustained. However, the difference are less extreme in the anonymized log, compared to the original log. This indicates that \emph{PRIPEL} is able to preserve the ability for such an analysis.

\begin{figure}[!htb]
	\centering
	\includegraphics[width=.95\columnwidth]{figures/sepsis_active_cases.pdf}
	\caption{Active Cases over Time}
	\label{fig:active_cases}
\end{figure}

To investigate the potential impact on other attributes with looked into the distribution of the attribute "InfectionSuspected". This attribute has a boolean value. We run the \emph{PRIPEL} framework with different values for $\epsilon$ to show its impact on he distribution of the attribute. The results are visualized in table~\ref{tab:sensitivity_attribute}. Based on this data we can see that distribution of the boolean values reaches a point of nearly complete randomness for $\epsilon=0.1$. While values above $\epsilon=1.0$ seem still to be able to preserve part of the original distribution. Therefore, we can conclude that maintaining utility seems possible for certain privacy levels.

\begin{table}
	\begin{tabularx}{\linewidth}{l X X X X X X}
		\toprule
		$\epsilon$&0.1 &0.5 & 1.0 & 1.5 & 2.0 & Original \\
		\midrule
		\% of  "True" & 0.51 & 0.58 &  0.67 & 0.69 & 0.75 & 0.81 \\
		%
		%
		\bottomrule
	\end{tabularx}
	\caption{Distribution of  "InfectionSuspected"  for different $\epsilon$}
	\label{tab:sensitivity_attribute}
\end{table}

\subsection{Discussion}
\label{sec:discussion}
With \emph{PRIPEL} we introduced an approach that is able to publish complete event logs, that fulfil differential privacy. Therefore, the anonymizied event log can be used, without violating modern privacy regulation such as the GDPR or CCPA.

However, our approach comes wit certain limitations and assumption. We need to assume, that one individual, such as a patient, is only represented in one case. Otherwise our differential privacy guarantee does not hold. Additionally, we assume that we can anonymize all attributes independently. This might not be possible to utility or privacy reasons. Some attributes might correlate strongly with each other, like the age and height of a child. If we anonymize them independently we might completely destroy the utility. Furthermore, if an attributes represents a measurement that appears several time in the trace, e.g. the weight of a person, anonymizing all measurements independently is harmful to the differential privacy guarantee. We also need to acknowledge that our approach to determine the sensitivity doe numerical attributes or timestamps is prone to outliers. Therefore, steps to reduce outliers might be a necessary preprocessing task to increase and maintain the utility of the anonymized log. Ultimately, it was proven in the past, that the utility of anonymized data is limited in a data mining setting\cite{brickell2008cost}. 

Besides these attribute related limitations our approach has additional limitations based on the trace-variant query. The size of the anonymized log can drastically differ from the original log. This can diminish the utility of the log in areas such as the analysis of bottlenecks. Additionally, we can not ensure that a behaviour present in the anonymized log, was part of the original log, contrary the \emph{PRETSA} algorithm can give such an guarantee. Furthermore, it is possible that a trace-variant-query deletes the most common trace-variant from the log. It is also possible, that the traces are obviously noise, e.g. if the release from an emergency rooms, happens before the arrival. Such obvious noise could be filtered out by an adversary. However, most of these issues could probably be tackled by more advanced trace-variant queries, than the current state-of-the-art.


\iffalse
		An incomplete list of limitations  of our approach
		\begin{enumerate}
			\item Assume that every individual is only represented in one case. Otherwise our guarantee does not hold
			\item Assume that we can anonymize the attributes independently. That might not be reasonable e.g. height and weight of humans usually correlates.
			\item We assume that each attribute appears independently and is  for example not a sequence of measurements like blood pressure. Otherwise our guarantee does not hold
			\item It could be, that traces can be perfectly matched. E.g. the trace variant query produces just additional noisy traces. This  could negatively impact the privacy of individual
			\item We could delete the most typical behaviour of the process and end up with total crap --> That is not possible with PRETSA
			\item We can not guarantee that behaviour in the anonymized  log is present in  the real world
			\item Our sensitivity-setting is prone to outliers in the distribution of attributes (local sensitivity could be a fix)
			\item The noise we add in terms of trace variants could be obviously noise and therefore filtered out by an adversary (E.g. Release from ER before Admission)
			\item The number of traces in the  original log can differ dramatically from the original log
			\item Our utility is limited by the cost of utility\ref{costOfUtility}
		\end{enumerate}
	
	\begin{enumerate}
		\item Different privacy guarantee, that does require about the background knowledge of an adversary. Contrary to  PRETSA and in $k$-anonymity in general.  \todo{Han: I'm sorry I still don't understand what you mean, probably also because there seems to be part of the sentence missing}
		\item Different $\epsilon$ for each attribute possible, based on privacy risk. Therefore, an additional level flexibility regarding the anonymization strength is given.
		\item Does not have to eliminate all outliers. Therefore, the detection of loop, with highly varying iteration number, is possible. 
		\todo{Han: this is more a feature depending on a discovery algorithm, right?}
		\item Minimal noise-level can be really fine tuned, while the minimal impact of PRETSA can be quite large. This is due to the fact, that $\epsilon$ is tuned as a real-number, while $k$ is an integer. However, this effect is especially true for business processes with a long tail.  
		\item Control-flow behaviour in anonymized log must not be part of original log, since it could be just noise, that was introduced. Therefore, plausible deniability is guaranteed. \todo{Han: do you mean ``was not necessarily part of the original log''? Currently it state that nothing in the anonymized log was in the original one}
		\item Mean of attributes should be close to original mean, therefore certain analytics such as performance analysis(e.g. for different variants) should be possible with high-utility. While PRETSA could highly influence the mean, since the deletion of duration data is not only guided based on the duration distribution, but also the distribution of control-flow behaviour. 
		\item Predictive process monitoring is possible, with well known utility cost\cite{brickell2008cost}. While a log anonymized with PRETSA could only be trained on a  projection of the  original log, that would disregard all other attributes.
		\item Can be used in a streaming/batching setting (finished traces are added in batches), since anonymization is on trace level, while PRETSA works in dataset level. However, the effect should be studied in detail, because I think known trace-variant-query mechanism are not well suited for this approach.
	\end{enumerate}
	
	I dissucessed with Dirk that a foundations paper would need the following things
	
	\begin{enumerate}
		\item Novel approach, that can  do something, that was not able before (check)
		\item We must show that our approach can work for all event logs
		\item We must show the feasibility  of our approach (see case study section) (check)
		\item We must discuss potential limitations  of our approach. This can not be done empirical, but must be done in a generalized manner-
		\item Han and I agreed looking into: runtime as a form of feasibility, showing the impact of our  approach compared to  the  original log, based on  one case study. Providing  a discussion regarding the limitations of our approach(e.g. cost of privacy). (partly check)
	\end{enumerate}

	
\fi
